From Stance to Concern: Adaptation of Propositional Analysis to New Tasks and Domains

We present a generalized paradigm for adaptation of propositional analysis (predicate-argument pairs) to new tasks and domains. We leverage an analogy between stances (belief-driven sentiment) and concerns (topical issues with moral dimensions/endorsements) to produce an explanatory representation. A key contribution is the combination of semi-automatic resource building for extraction of domain-dependent concern types (with 2-4 hours of human labor per domain) and an entirely automatic procedure for extraction of domain-independent moral dimensions and endorsement values. Prudent (automatic) selection of terms from propositional structures for lexical expansion (via semantic similarity) produces new moral dimension lexicons at three levels of granularity beyond a strong baseline lexicon. We develop a ground truth (GT) based on expert annotators and compare our concern detection output to GT, to yield 231% improvement in recall over baseline, with only a 10% loss in precision. F1 yields 66% improvement over baseline and 97.8% of human performance. Our lexically based approach yields large savings over approaches that employ costly human labor and model building. We provide to the community a newly expanded moral dimension/value lexicon, annotation guidelines, and GT.

==> Attic/old-comments.tex <==

concern type induction

\owen{I think since the results are low, we need to do an error analysis.  While it is great that our techniques can increase R (as we would expect) without hurting P (or only a teensy bit), the fact of the matter is that this precision is low.  Our lexicon-based method is making too many predictions.  There are 66 correct predictions, but we are making 224, which is why we have low precision.  Why is that?  Is this an intrinsic problem of our approach (presumably not).  Do we have an idea of how to improve this in future work?}


moral value expansopn

\owen{Same comment as above -- are we presenting a general algo or describing what we did for this dataset (with teh udnerstanding that it generalizes)?}
